Brick-DICL: Dynamic In-Context Learning for Automated Brick Schema Classification

Building Management Systems (BMS) are essential for optimizing energy efficiency and operational performance in modern buildings. However, the lack of standardization across BMS points from different manufacturers creates significant barriers to integration and data utilization. While the Brick schema offers a standardized ontology for building systems, mapping BMS points to appropriate Brick classes presents three critical challenges: (i) the extensive number of Brick classes (936 in the latest version), (ii) limited domain-specific knowledge in large language models (LLMs), and (iii) substantial manual effort required for verification. To address these challenges, we propose Brick-DICL, a two-stage dynamic in-context learning framework for automated Brick schema classification. Brick-DICL consists of two primary components: metadata-RAG, which retrieves relevant examples to enhance LLMs' domain knowledge, and class-RAG, which narrows down potential Brick classes to address the large classification space. Additionally, we implement a multi-LLM filtering mechanism that compares predictions across multiple models, flagging low-confidence classifications for human review. As a result: (i) General: Brick-DICL is applicable to any building management system regardless of manufacturer or metadata format; (ii) Novel and Powerful: as the first dynamic in-context learning approach for Brick schema classification, Brick-DICL achieves significant classification accuracy improvements on building datasets, outperforming existing methods; (iii) Efficient: our multi-LLM filtering strategy reduces manual verification effort, enabling rapid digital building onboarding. Extensive experiments demonstrate Brick-DICL's effectiveness across diverse building datasets, accelerating the path toward standardized, interoperable building management systems.

==> section/acknowledge.tex <==
\section{Acknowledgement}
This work was partially conducted during my internship, where I received invaluable guidance and support. I would like to express my gratitude to my colleagues from that period. I also wish to thank my current GenAIIC team  for their continued support and for providing the resources and environment necessary to extend this work. Their encouragement and insights have been instrumental in bringing this work to fruition.

==> section/statement.tex <==
\section*{Customer Problem Statement}
\vspace{-0.1in}
As AWS customers in the building management system industry increasingly seek generative AI solutions to automate and standardize the onboarding of diverse building data, it has become essential to develop robust frameworks that address the unique challenges of this domain. The growing complexity and heterogeneity of BMS metadata, spanning thousands of points across equipment, sensors, and control systems, make manual mapping to standardized ontologies like Brick both time-consuming and error-prone. There is immediate demand for solutions that can accelerate digital transformation, reduce operational costs, and enable scalable analytics for building owners, operators, and service providers. Our work responds directly to these customer needs by advancing retrieval-augmented, dynamic in-context learning, and multi-LLM consensus strategies for BMS point classification. This not only delivers immediate value by streamlining digital onboarding and normalization of building data, but also lays the groundwork for long-term adoption of automated, AI-driven semantic modeling and management in the smart building sector.


